SPD-DDPM: Denoising Diffusion Probabilistic Models in the Symmetric Positive Definite Space

Symmetric positive definite~(SPD) matrices have shown important value and applications in statistics and machine learning, such as FMRI analysis and traffic prediction. Previous works on SPD matrices mostly focus on discriminative models, where predictions are made directly on $E(X|y)$, where $y$ is a vector and $X$ is an SPD matrix. However, these methods are challenging to handle for large-scale data, as they need to access and process the whole data. In this paper, inspired by denoising diffusion probabilistic model~(DDPM), we propose a novel generative model, termed SPD-DDPM, by introducing Gaussian distribution in the SPD space to estimate $E(X|y)$. Moreover, our model is able to estimate $p(X)$ unconditionally and flexibly without giving $y$. On the one hand, the model conditionally learns $p(X|y)$ and utilizes the mean of samples to obtain $E(X|y)$ as a prediction. On the other hand, the model unconditionally learns the probability distribution of the data $p(X)$ and generates samples that conform to this distribution. Furthermore, we propose a new SPD net which is much deeper than the previous networks and allows for the inclusion of conditional factors. Experiment results on toy data and real taxi data demonstrate that our models effectively fit the data distribution both unconditionally and unconditionally and provide accurate predictions.

==> body/approment.tex <==
\section{Approment}

\subsection{Operation in SPD Space}

In this section, we will derive some operational properties in the SPD space, which will help us deduce properties of denosing diffusion probability model.

\subsubsection{Distributive Law of Multiplication}

Suppose $a$ is a scale,$X,Y$ are SPD matrices. Then 
\begin{equation}%加*表示不对公式编号
	a \odot (X \oplus Y) = a \odot X \oplus a \odot Y.\label{distribute law}
\end{equation}

Proof:
\begin{equation*}%加*表示不对公式编号
	\begin{split}
		a \odot (X \oplus Y) &= a \odot exp(logX+logY)\\
		&= exp[a \cdot log(exp(logX +logY))]\\
		&= exp[a \cdot(logX +logY)]\\
		&= exp[alogX +alogY]\\
		&= exp[log[exp(alogX)]+log[exp(alogY)]]\\
		&= exp[alogX]\oplus exp[alogY]\\
		&= a \odot X \oplus a \odot Y. 
	\end{split} 
\end{equation*}


\subsubsection{Combining Similar Terms}

Suppose $a,b$ is a scale, $X$ is a SPD materic. Then 

\begin{equation}%加*表示不对公式编号
	a \odot X \oplus b \odot X = (a+b)\odot X.\label{conbine}
\end{equation}

Proof: 
\begin{equation*}%加*表示不对公式编号
	\begin{split}
		&a \odot X \oplus b \odot X \\
		&= exp(alogX) \oplus exp(blogX)\\
		&= exp[log(exp(alogX))+log(exp(blogX))]\\
		&= exp[alogX+blogX]\\
		&= exp[(a+b)logX]\\
		&= (a+b) \odot X.  
	\end{split}
\end{equation*}

\subsubsection{Multiplication of Gussian Distribution in SDP Space}

Suppose $a$ is a scale, $\epsilon_t \sim G(E,\sigma_t^2)$, Then  
\begin{equation}%加*表示不对公式编号
	a \odot \epsilon_t \sim G(E,a^2\sigma_t^2). \label{multiplication}
\end{equation}

Proof:
\begin{equation*}%加*表示不对公式编号
	\begin{split}
		d(\epsilon_t^a,E)^2 &= tr[log\epsilon_t^a]^2 = tr[alog\epsilon_t]^2 = a^2tr[log\epsilon_t]^2\\
		P(d(\epsilon_t^a,E) &=P(d(\epsilon_t,E)^2<(\frac{r}{a})^2)\\
		&= \frac{\int_0^{\frac{r^2}{a^2}}e^{-\frac{u}{\sigma_t^2}}\,du}{\int_0^{\inf}e^{-\frac{u}{\sigma_t^2}}\,dz}\\
		&= \frac{\int_0^{r^2}e^{-\frac{z}{\sigma_t^2a^2}}\,du}{\int_0^{\inf}e^{-\frac{z}{\sigma_t^2a^2}}\,dz}\\
		& \sim G(E,a^2\sigma_t^2). 
	\end{split}
\end{equation*}

\subsubsection{Constant Plus of Gussian Distribution in SPD Space}

Suppose $Y$ is a constant SPD matrice, $\epsilon \sim G(E,\sigma^2)$. Then 
\begin{equation}%加*表示不对公式编号
	Y \oplus \epsilon \sim G(Y, \sigma^2).\label{constant plus} \quad \eqref{transforamtion}
\end{equation}

Proof:
\begin{equation*}%加*表示不对公式编号
	\begin{split}
		Y \oplus \epsilon &= exp[logY+log\epsilon]\\
		&= exp[\frac{1}{2}logY +log\epsilon +\frac{1}{2}logY] \\
		&= Y^{\frac{1}{2}}\epsilon Y^{\frac{1}{2}}\\
		& \sim G(Y,\sigma^2).
	\end{split}
\end{equation*}

\subsubsection{Plus of Gussian Distribution in SPD Space}
Suppose $\epsilon_1 \sim G(E,\sigma_1^2)$, $\epsilon_2 \sim G(E,\sigma_2^2)$. Then
\begin{equation}%加*表示不对公式编号
	\epsilon_1 \oplus \epsilon_2 \sim G(E,\sigma_1^2+\sigma_2^2). \label{plus of gussian distribution}
\end{equation}

Proof:

$Define \quad Z = \epsilon_1 \oplus \epsilon_2$

\begin{equation*}%加*表示不对公式编号
	\begin{split}
		&P(Z = a) \\
		&= \int_M p(\epsilon_1 = b)p(\epsilon_2 = a\ominus b ) \,dv(b)\\
		&= \inf_M \frac{1}{\zeta(\sigma_1)}\frac{1}{\zeta{\sigma_2}} exp[-\frac{d(E,b)^2}{2\sigma_1^2}-\frac{d(E,a \ominus b)^2}{2 \sigma_2^2}] \,dv(b)\\
		&= \int_M \frac{1}{\zeta(\sigma_1)} \frac{1}{\zeta({\sigma_2})} exp[\\
		&\qquad -\frac{(\sigma_1^2+\sigma_2^2)tr[logb]^2}{2\sigma_1^2 \sigma_2^2}\\
		&\qquad \frac{-2\sigma_1^2tr[logalogb]+\sigma_1^2tr[loga]^2}{2\sigma_1^2 \sigma_2^2}]\,dv(b)\\
		&= \int_M \frac{1}{\zeta(\sigma_1)} \frac{1}{\zeta({\sigma_2})} exp[\\
		&\qquad -\frac{tr[\sqrt{\sigma_1^2+\sigma_2^2}logb-\frac{\sigma_1^2}{\sqrt{\sigma_1^2+\sigma_2^2}}loga]^2}{2\sigma_1^2\sigma_2^2}\\
		&\qquad+\frac{[\sigma_1^2-\frac{\sigma_1^4}{\sigma_1^2+\sigma_1^2}]tr[loga]^2}{2\sigma_1^2\sigma_2^2}]\,dv(b)\\
		&= exp[-\frac{1-\frac{\sigma_1^2}{\sigma_1^2+\sigma_2^2}}{2\sigma_2^2}tr[loga]^2]\frac{1}{\zeta(\sigma_1)} \frac{1}{\zeta(\sigma_2)} \\
		&\qquad\int_M  exp[-\frac{tr[\sqrt{\sigma_1^2+\sigma_2^2}logb-\frac{\sigma_1}{\sqrt{\sigma_1^2+\sigma_2^2}}loga]^2}{2\sigma_1^2\sigma_2^2}]dv(b)\\
		&\propto \, exp[-\frac{d(E,a)^2}{2(\sigma_1^2+\sigma_2^2)}].
	\end{split} 
\end{equation*}

\subsubsection{Distance of matrix power}
Suppose $A$ and $B$ are SPD matrices, a is a scale. Then 

\begin{equation}%加*表示不对公式编号
	d(A^a,B^a)^2 = \sqrt{a}\,d(A,B)^2. \label{distance of matrix power}
\end{equation}

Proof:

\begin{equation*}%加*表示不对公式编号
	\begin{split}
		d(A^a,B^a)^2 &= tr[logA^{-\frac{a}{2}}B^aA^{-\frac{a}{2}}]^2\\
		&= tr[-\frac{a}{2}logA \oplus alogB \oplus-\frac{a}{2}logA]^2\\
		&= \sqrt{a}tr[-\frac{1}{2}logA \oplus logB \oplus-\frac{1}{2}logA]^2\\
		&= \sqrt{a} tr[logA^{-\frac{1}{2}}BA^{-\frac{1a}{2}}]^2\\
		&= d(A,B)^2.
	\end{split} 
\end{equation*}


\subsection{Reparameterization of $q(x_t|x_0)$}

If $q(x_t|x_{t-1}) \sim G(\alpha_t \odot x_{t-1}, \sigma_t^2)$,  $x_t$ can be written as:
\begin{equation*}%加*表示不对公式编号
	\begin{split}
		x_t = \alpha_t \odot x_{t-1} \oplus \epsilon_t.
	\end{split}
\end{equation*}

This can be This can be further promoted as:

\begin{equation}%加*表示不对公式编号
	\begin{split}
		x_t &= \alpha_t \odot x_{t-1} \oplus \epsilon_t\\
		&= \alpha_t \odot (\alpha_{t-1} \odot x_{t-2} \oplus \epsilon_{t-1})\oplus \epsilon_t\\
		&= \alpha_t \alpha_{t-1}\odot x_{t-2} \oplus \alpha_t \odot \epsilon_{t-1} \oplus \epsilon_t \quad follow \;\eqref{distribute law} \\
		&= (\alpha_t\dots \alpha_1)\odot x_0 \oplus (\alpha_t \dots \alpha_2)\sigma_1 \epsilon_1 \oplus \dots \oplus \alpha_t \sigma_t \epsilon_t \oplus \sigma_t\epsilon_t\\
		&= \bar{\alpha}_t \odot x_0 +\sqrt{1-\bar{\alpha}_t^2} \odot \bar{\epsilon}_t, \, \bar{\epsilon}_t \sim G(E,1) \quad follow \;\eqref{plus of gussian distribution}\\
		&\sim G(\bar{\alpha}_t,1-\bar{\alpha}_t^2). \quad follow \;\eqref{constant plus} \eqref{multiplication}
	\end{split} \label{x_tx_0}
\end{equation}


\subsection{Computation of $q(x_{t-1}|x_t,x_0)$}

\begin{equation*}%加*表示不对公式编号
	\begin{split}
		&q(x_t|x_{t-1},x_0) \\
		&= q(x_t|x_{t-1})\frac{q(x_{t-1}|x_0)}{q(x_t)|x_0}\\
		&= G(\alpha_t \odot x_{t-1},\sigma_t) \frac{G(\bar{\alpha}_{t-1} \odot x_0, \bar{\sigma}_{t-1})}{G(\bar{\alpha}_{t} \odot x_0, \bar{\sigma}_{t}}\\
		& = \frac{\zeta(\bar{\sigma}_t)}{\zeta(\sigma_t)\zeta(\bar{\sigma}_{t-1})} exp(-\frac{d(x_t,x_{t-1}^{\alpha_{t}})^2}{2 \sigma_t^2} \\
		&\qquad -\frac{d(x_{t-1},x_0^{\bar{\alpha}_{t-1}})}{2\bar{\sigma}_{t-1}^2}-\frac{d(x_{t},x_0^{\bar{\alpha}_{t}})}{2\bar{\sigma}_{t^2}})\\
		& \propto exp(-\frac{d(x_t,x_{t-1}^{\alpha_{t}})^2}{2 \sigma_t^2}-\frac{d(x_{t-1},x_0^{\bar{\alpha}_{t-1}})}{2\bar{\sigma}_{t-1}^2})\\
		& = exp(-\frac{\bar{\sigma}_{t-1}^2 d(x_t,x_{t-1}^{\alpha_{t}})^2+\sigma_{t}^2 d(x_{t-1},x_0^{\bar{\alpha}_{t-1}})}{2\sigma_t^2 \bar{\sigma_{t-1}}^2})\\
		& = exp(-\frac{\bar{\sigma}_{t-1} tr[log(x_t^{-\frac{1}{2}}x_{t-1}^{\alpha_t}x_t^{-\frac{1}{2}})]^2}{2\sigma_t^2 \bar{\sigma_{t-1}}^2}+\\
		&\qquad\frac{\sigma_{t}^2tr[log( x_0^{-\frac{\bar{\alpha}_{t-1}}{2}} x_{t-1} x_0^{-\frac{\bar{\alpha}_{t-1}}{2}})]^2}{2\sigma_t^2 \bar{\sigma_{t-1}}^2})\\
		& = exp(\frac{tr[\bar{\sigma}_{t-1}^2 log(x_t^{-\frac{1}{2}}x_{t-1}^{\alpha_t}x_t^{-\frac{1}{2}})}{2\sigma_t^2 \bar{\sigma_{t-1}}^2}+\\
		&\qquad	\frac{\sigma_{t}^2log( x_0^{-\frac{\bar{\alpha}_{t-1}}{2}} x_{t-1} x_0^{-\frac{\bar{\alpha}_{t-1}}{2}})]^2}{2\sigma_t^2 \bar{\sigma_{t-1}}^2}).
	\end{split}
\end{equation*}

Translate $A = x_t^{-\frac{1}{2}}$ ,$B = x_{t-1}$, $C = x_0^{-\frac{\bar{\alpha}_{t-1}}{2}}$, $a = \bar{\sigma}_{t-1}$, $b = \sigma_t$, $r = \alpha_t$

Then the numerator can be written as:

\begin{equation}%加*表示不对公式编号
	\begin{split}
		&a^2(log AB^rA)^2 + b^2(logCBC)^2 \\
		& = a^2(logA+logB^r+logA)^2 \\
		& \qquad +b^2(logC+logB+logC)^2\\
		&= 4a^2(logA)^2 +a^2(logB^r)^2 +2a^2logAlogB^r\\
		& \qquad+2a^2logB^rlogA +4b^2(logC)^2+b^2(logB)^2\\
		& \qquad +2b^2logclogB+2b^2logBlogC\\
		&= (a^2r^2+b^2)(logB)^2 +2(a^2r logA+b^2 logC)logB \\
		&\quad+2logB(a^2 rlogA+b^2 logC)+4a^2(logA)^2 +4b^2(logC)^2\\
		&= (a^2r^2+b^2)[(logB)^2 + 2\frac{a^2rlogA+b^2logC}{a^2r^2+b^2}logB\\
		&\quad+2logB\frac{a^2rlogA+b^2logC}{a^2r^2+b^2}]+4a^2(logA)^2+4b^2(logC)^2\\
		& \propto(a^2r^2+b^2)(logD+logB+logD)^2\\
		&\qquad logD = \frac{a^2rlogA+b^2logC}{a^2r^2+b^2}\\
		&= (a^2r^2+b^2)(logDBD)^2\\
		&\qquad D = A^{\frac{a^2r}{2(a^2r^2+b^2)}}C^{\frac{b^2}{a^2r^2+b^2}}A^{\frac{a^2r}{2(a^2r^2+b^2)}}.	 
	\end{split}
\end{equation}

Thus $q(x_{t-1}|x_t,x_0)$ can be written as:

\begin{equation}%加*表示不对公式编号
	\begin{split}
		q(x_{t-1}|x_t,x_0) &\propto exp[-\frac{tr(a^2r^2+b^2)(logDBD)^2}{2\bar{\sigma}_{t-1}^2\sigma_t^2}]\\
		&= exp[-\frac{tr[logDBD]^2}{2\frac{\bar{\sigma}_{t-1}^2\sigma_t^2}{a^2r^2+b^2}}]\\
		&\sim G(\mu_t , \tilde{\sigma}_{t-1}^2),
	\end{split}
\end{equation}

\begin{equation*}%加*表示不对公式编号
	\tilde{\sigma}_{t-1}^2 =\frac{\bar{\sigma}_{t-1}^2\sigma_t^2}{a^2r^2+b^2} = \frac{\bar{\sigma}_{t-1}^2\sigma_t^2}{\bar{\sigma}_{t-1}^2\alpha_t^2+\sigma_t^2} = \frac{\bar{\sigma}_{t-1}^2\sigma_t^2}{\bar{\sigma}_t^2},
\end{equation*}


\begin{equation*}%加*表示不对公式编号
	\begin{split}
		\mu_t &= D^{-2} \\
		&=A^{-\frac{a^2r}{2(a^2r^2+b)}}C^{-\frac{b}{2^2(a^2r^2+b)}}A^{-\frac{a^2r}{2(a^2r^2+b)}}\\
		& \quad C^{-\frac{b}{2^2(a^2r^2+b)}}A^{-\frac{a^2r}{2(a^2r^2+b)}}\\
		&= x_t^{\frac{\bar{\sigma}_{t-1}^2 \alpha_t}{4(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)}} x_0^{\frac{\bar{\alpha}_{t-1}\sigma_t^2}{2(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)}}x_t^{\frac{\bar{\sigma}_{t-1}^2 \alpha_t}{4(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)}}\\ 
		& \quad x_0^{\frac{\bar{\alpha}_{t-1}\sigma_t^2}{2(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)}}x_t^{\frac{\bar{\sigma}_{t-1}^2 \alpha_t}{4(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)}}\\
		&= \frac{\bar{\sigma}_{t-1}^2 \alpha_t}{(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)} \odot x_t \oplus \frac{\bar{\alpha}_{t-1}\sigma_t^2}{(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)} \odot x_0\\
		&= \frac{\bar{\sigma}_{t-1}^2 \alpha_t}{(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)} \odot x_t \\
		&\quad \oplus \frac{\bar{\alpha}_{t-1}\sigma_t^2}{(\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2)} \odot [\frac{1}{\bar{\alpha}_t}(x_t \ominus \sqrt{\alpha_t^2\bar{\sigma}^2_{t-1}+\sigma_t^2}\epsilon_t]\\
		&= \frac{\sigma_t^2+\alpha_t^2\bar{\sigma}^2_{t-1}}{\alpha_t(\alpha_{t}^2\bar{\sigma}_{t-1}^2+\sigma_t^2)} \odot x_t \ominus \frac{\sigma_t^2}{\alpha_t \sqrt{\alpha_{t}^2\bar{\sigma}_{t-1}^2+\sigma_t^2}} \odot \epsilon_t\\
		&= \frac{1}{\alpha_t} \odot x_t \ominus\frac{\sigma_t^2}{\alpha_t \bar{\sigma}_t} \odot \epsilon_t.
	\end{split}
\end{equation*}


\subsection{Loss Function}
Assume
\begin{equation*}%加*表示不对公式编号
	\begin{split}
		&q(x_{t-1}|x_t,x_0) \sim G(\mu_1,\sigma_1)\\
		&p(x_{t-1}|x_t) \sim G(\mu_2, \sigma_2),
	\end{split}
\end{equation*}
Then their KL divergence can be bounded by:

\begin{equation}%加*表示不对公式编号
	\begin{split}
		&KL(q(x_{t-1}|x_t,x_0) \parallel p(x_{t-1}|x_t)) \\
		&\propto \frac{2\sigma_1^2d(\mu_2,x)^2-2\sigma_2^2d(\mu_1,x)}{2\sigma_1^2\sigma_2^2}\\
		& \propto \frac{2\sigma_1^2[d(\mu_2,x)^2-d(\mu_1,x)^2]}{2\sigma_1^2\sigma_2^2}\\
		& \le d(\mu_1,\mu_2)^2.\label{kl}
	\end{split}
\end{equation}

==> body/proof_pro1.tex <==
\section{Proof of Proposition 1}
\begin{proposition}
    \label{transformation}
    $X \sim G(\bar{X},\sigma^2) \implies X\cdot A \sim G(\bar{X} \cdot A,\sigma^2).$
\label{pro_1}
\end{proposition}
Proof:

For any function $f:P_m \rightarrow R$ ($P_m$ is SPD space), and any $A \in GL(m)$, we have(according to Eq.14 in main paper):
\begin{equation*}%加*表示不对公式编号
    \int_{P_m} f(X) dv(X) = \int_{P_m} f(X \cdot A)dv(X).
\end{equation*}
where $dv(X)$ is the Riemannian volume element defined as:

\begin{equation*}%加*表示不对公式编号
    dv(X) = det(X)^{-\frac{m+1}{2}} \prod_{i\le j}dX_{ij}.
\end{equation*}
Intuitively, $dv(X)$ is the Riemannian volume element of $ds^2(X)$, and $ds^2(X)$ is invariant under congruence transformations and inversion:
\begin{equation*}%加*表示不对公式编号
    ds^2(X) = tr[X^{-1}dX]^2.
\end{equation*}

Let $X$ be a random variable in $P_m$, let $\phi:P_m \rightarrow R$ be a test function. If $X\sim G(\bar{X},\sigma^2)$ and $Z=X \cdot A$, then the expection of $\phi(Z) $is given by:
\begin{equation*}%加*表示不对公式编号
\begin{split}
    &\int_{P_m} \phi(X \cdot A)p(X|\bar{X},\sigma^2)dv(X) \\
    &=\int_{P_m}\phi(Z)p(Z \cdot A^{-1}|\bar{X},\sigma^2)dv(Z)\\
    &=  \int_{P_m}\phi(Z)p(Z|\bar{X}\cdot A,\sigma^2)dv(Z).
\end{split}
\end{equation*}
